Causal Embeddings for Recommendation: An Extended Abstract

Recommendations are commonly used to modify user's natural behavior, for example, increasing product sales or the time spent on a website. This results in a gap between the ultimate business objective and the classical setup where recommendations are optimized to be coherent with past user behavior. To bridge this gap, we propose a new learning setup for recommendation that optimizes for the Incremental Treatment Effect (ITE) of the policy. We show this is equivalent to learning to predict recommendation outcomes under a fully random recommendation policy and propose a new domain adaptation algorithm that learns from logged data containing outcomes from a biased recommendation policy and predicts recommendation outcomes according to random exposure. We compare our method against state-of-the-art factorization methods, in addition to new approaches of causal recommendation and show significant improvements.

==> 3-our_approach.tex <==
%----------------------------------------------------------------------------------------
%	SECTION - Proposed Approach
%----------------------------------------------------------------------------------------
\section{Proposed Approach}
\label{sec:proposedapproach}

As discussed in Section \ref{sec:intro}, we are interested in building a good predictor for recommendation outcomes under random exposure for all the user-product pairs, which we denote as $\hat{y}_{ij}^{rand}$. In our learning setup, we assume that we have access to a large sample $S_c$ from the logging policy $\pi_c$ and a small sample $S_t$ from the randomized treatment policy $\pi_t^{rand}$. To this end, we propose a multi-task objective that jointly factorizes the matrix of observations $y^c_{ij} \in S_c$ and the matrix of observations $y^t_{ij} \in S_t$.

\subsection{Multi-Task Objective For Exposure Policies That Vary Treatments For A Given Set Of Fixed Users}
For simplicity we assume that the same set of users are exposed differently in control/treatment and the exposure change between treatment and control is explained by the difference in product representations in the two policies. In this case, \emph{the users have a fixed representation (either as a set of user features or as a user embedding vector)}. This is the evaluation setup proposed in \cite{liangcausal} and the equivalent evaluation of the work in \cite{schnabel2016recommendations}, where the test sample is produced according to $\pi^{rand}_t$.

The case of predicting outcomes under changing treatment exposures for the same set of users is also addressed by the authors in \cite{rosenfeld2016predicting}. They assume a user-independent exposure policy and derive a multi-task objective that explains jointly the small sample $S_t$ and the big sample $S_c$ and regularizes the difference in the two resulting product representations. In order to motivate this objective, the authors assume that both the expected factual control and treatment rewards can be approximated as linear predictors over the fixed user representations $u_i$:
\begin{equation}
\begin{split}
y^{c}_{ij} \approx <\theta^{c}_j,u_i>\\
y^{t}_{ij} \approx <\theta^{t}_j,u_i>
\end{split}
\end{equation}
where $\theta^{c}_j,\theta^{t}_j$ are the control/treatment vectorial representations of product $j$ and $< x , y >$ denotes the inner product between the vectors $x$ and $y$.

As a result and using the logic of Equation \ref{eq:itepair}, we can approximate the ITE of a user-product pair $i,j$ as the difference between the two:
\begin{equation}
\widehat{ITE}_{ij} = <\theta^t_j,u_i> - <\theta^c_j,u_i> = <\theta^{\Delta}_j, u_i>
\end{equation}

We define the first part of our joint prediction objective as the supervised predictor for $y^t_{ij}$, trained on the limited sample $S_t$. We denote the associated loss term by $l^t_{ij}$:
\begin{equation}
l^t_{ij} =  L(<\theta^t_j, u_i>, y^t_{ij}) + \Omega(\theta^t_j)
\end{equation}

where: $L$ is an arbitrary loss function and and $\Omega(.)$ is a regularization term over the weights of the model.
Switching to matrix notation, we define the associated objective by $L_t$:
\begin{equation}
\label{eq:lt}
L_{t} = \sum_{(i,j,y_{ij}) \in S_t} l^t_{ij} = L(U \Theta_t  , Y_t) + \Omega(\Theta_t)
\end{equation}

where $\Theta_t$ is the parameter matrix of treatment product representations, $U$ is the fixed matrix of the user representations, $Y_t$ is the observed rewards matrix, $L(.)$ is an arbitrary loss function and $\Omega(.)$ is a regularization term over the weights of the model.

Then, if we want to leverage the ample control data, we can use our treatment product representations by subtracting $ \theta^{\Delta}_j$ since $<\theta^c_j,u_i> = <\theta^t_j,u_i>  - <\theta^{\Delta}_j, u_i>$. We denote the associated objective by $l^{c}_{ij}$:
\begin{equation}
l^c_{ij} = L(<\theta^t_j - \theta^{\Delta}_j, u_i>, y^{c}_{ij}) + \Omega(\theta^t_j) + \Omega(\theta^{\Delta}_j) 
\end{equation}
If instead of parametrizing it in terms of treatment embeddings $\theta^t_j$ and a set of difference vectors $\theta^{\Delta}_j$, we choose to express the loss in terms of the new control embedding $\theta^c_j$, and switching to matrix notation, we have that:

\begin{equation}
\label{eq:lc}
\begin{split}
L_{c} = L(U \Theta_c  , Y_c) + \Omega(\Theta_c) + \Omega(\Theta_t - \Theta_c)
\end{split}
\end{equation}

By putting the two tasks together (eq. \ref{eq:lt} and \ref{eq:lc}), we have the equation of the joint tasks loss $L^{prod}_{CausE}$:
\begin{equation}
\label{eq:prod}
\begin{split}
L^{prod}_{CausE}= \underbrace{L(U \Theta_t  , Y_t) + \Omega(\Theta_t)}_{treatment~task~loss} +  \underbrace{L(U \Theta_c  , Y_c) + \Omega(\Theta_c)}_{control~task~loss} + \\ + \underbrace{\Omega(\Theta_t - \Theta_c)}_{regularizer~between~tasks}
\end{split}
\end{equation}
We can similarly define $L^{user}_{CausE}$, where the user embeddings are learnt over fixed product representations. This type of modelization is relevant for the cases where we know that the treatment policy differs from the control policy in terms of the choice of users.



\subsubsection{Optimization}
We optimize $L_{CausE}$ using Stochastic Gradient Descent (SGD) with momentum \cite{sutskever2013importance} and a linearly decaying learning rate. For our experiments we optimize $L^{prod}_{CausE}$ since our treatment policy depends only on products and not on users. Algorithm \ref{algo:cause} details the general \emph{CausE} method.

\begin{algorithm}[h]

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

 \Input{Mini-batches of $S_c = { \{ (u^c_i, p^c_j, \delta^c_{ij}) \} }^{M_c}_{i=1}$ and $S_t = { \{ (u^t_i, p^t_j, \delta^t_{ij}) \} }^{M_t}_{i=1}$ , regularization parameters $\lambda_{t},\lambda_{c}$ for the two joint tasks $L_t$ and $L_c$ and $\lambda_{dist}$ the regularization parameter for the discrepancy between the two representations for products and users, learning rate $\eta$}

 \Output{$\Gamma_t, \Gamma_c, \Theta_t, \Theta_c$ - User and Product Control and Treatment Matrices} 
 Random initialization of $\Gamma_t, \Gamma_c, \Theta_t, \Theta_c$ \;
 \While{not converged}{
  Read batch of training samples\;
      \For{\textbf{each} training sample $s$ in the batch:}{
	  		\If{$s \in S_c$}{	
	  			Lookup the product index $j$ and user index $i$ in $\Theta_c, \Gamma_c$ and \\
	  			Update control product vector: $\theta^c_j \leftarrow \theta^c_j - \eta \nabla L^{prod}_{CausE}$ \\ 
	  			Update control user vector: $\gamma^c_i \leftarrow \gamma^c_i - \eta \nabla L^{user}_{CausE}$ 
	  		}    
	  		\If{$s \in S_t$}{	 
	  			Lookup the product index $j$ and user index $i$ in $\Theta_t, \Gamma_t$ and \\
	  			Update treatment product vector: $\theta^c_j \leftarrow \theta^c_j - \eta \nabla L^{prod}_{CausE}$ \\
	  			Update treatment user vector: $\gamma^c_i \leftarrow \gamma^c_i - \eta \nabla L^{user}_{CausE}$ 
	  		}        
	  	}
   }
   \Return{$\Gamma_t, \Gamma_c, \Theta_t, \Theta_c$}
 \caption{CausE Algorithm: Causal Embeddings For Recommendations}
 \label{algo:cause}
\end{algorithm}


%\subsubsection{Multi-task Objective For Exposure Policies that Vary Both Treatments And Users}
%In this case, the change in exposure between treatment and control is explained both by the different choice in exposed users and products shown. To this end, we modify our objective function to allow for the user representations to change, and using similar reasoning to eq (\ref{eq:prod})  we reach $L_{CausE}$, the final loss function for our method:
%We can recover the previous loss as a special case by setting the regularization parameter on the difference between treatment and control representations for users to infinity.
